Fine-grained Human Activity Recognition Using Virtual On-body Acceleration Data

Previous work has demonstrated that virtual accelerometry data, extracted from videos using cross-modality transfer approaches like IMUTube, is beneficial for training complex and effective human activity recognition (HAR) models. Systems like IMUTube were originally designed to cover activities that are based on substantial body (part) movements. Yet, life is complex, and a range of activities of daily living is based on only rather subtle movements, which bears the question to what extent systems like IMUTube are of value also for fine-grained HAR, i.e., When does IMUTube break? In this work we first introduce a measure to quantitatively assess the subtlety of human movements that are underlying activities of interest--the motion subtlety index (MSI)--which captures local pixel movements and pose changes in the vicinity of target virtual sensor locations, and correlate it to the eventual activity recognition accuracy. We then perform a "stress-test" on IMUTube and explore for which activities with underlying subtle movements a cross-modality transfer approach works, and for which not. As such, the work presented in this paper allows us to map out the landscape for IMUTube applications in practical scenarios.

==> figure/low_mid_high_real.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{c c}
    \includegraphics[width=.45\linewidth]{figure/low_mid_high_real/low_macro_f1.pdf} &  
    \includegraphics[width=.45\linewidth]{figure/low_mid_high_real/mid_macro_f1.pdf}\\
    \includegraphics[width=.45\linewidth]{figure/low_mid_high_real/high_macro_f1.pdf} &
    \includegraphics[width=.45\linewidth]{figure/low_mid_high_real/coresponding_data_to_motion.pdf}
    \end{tabular}
    \caption{Within MSI-group classification performance with varying size of real IMU dataset for model training.
    For each case, we also compared the model performance with when using all virtual IMU dataset ignoring MSI.
    For the reference, we also included classification performance with all activity classes with the proposed method (bottom right).
    % \hyeok{please remove real+low/high the old result from this figure.}
    }
    \label{fig:low_mid_high_real}
\end{figure}

==> figure/msi_corr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.95\linewidth]{figure/real_optical.pdf}
    \caption{Pearson correlation Analysis between MSI and rMSI modes from distributions for all classes in daily activity dataset~\cite{inproceedings}. 
    Strongly positive correlation existed between the MSI and rMSI values across 17 activities ($r=0.746$, $p\leq 0.006$) validating MSI as an objective metric for quantifying subtle motions in activities.
    }
    \label{fig:msi_corr}
\end{figure}

==> figure/msi_f1_spline.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/daily_activity/msi_f1_20_spline.pdf}
    \caption{Spline curve fitting with MSI vs F1 score change for each class.
    MSI values are calculate from the mode of MSI distribution for each class.
    Most positive F1 score change was observed in classes with $0.35 \leq MSI \leq 3.33$.
    }
    \label{fig:msi_f1_spline}
\end{figure}

==> figure/msi_vs_f1.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c}
    Daily Activity & \hl{Eating} \\
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/all_activities_f1.pdf} &  
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/all_activities_f1.pdf}
    \end{tabular}
    \caption{Classification performance changes according to MSI values for Virtual IMU data. The values in X-axis are the upper threshold value for including virtual IMU data according to MSI values.
    Y-axis is the changes in F1 score compared to the baseline model that only uses real IMU data for model training.
    \hyeok{Waiting for Zikang to generate Eating figure}
    }
    \label{fig:msi_f1}
\end{figure}

==> figure/msi_vs_f1_per_class.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c}
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/Eat_with_hand.pdf} & 
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/Driving_Automatic.pdf} \\
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/Flipping.pdf} &
    \includegraphics[width=.45\linewidth]{figure/msi_vs_f1/Washing_Hands.pdf}
    \end{tabular}
    \caption{Per-class classification performance change according to MSI values.
    Eating and driving automatic falls into low MSI category, flipping falls into mid MSI category, and washing hands falls into high MSI category.
    The most effective MSI value depends on the underlying activity showing that low MSI activity prefers low MSI threshold and vice versa.
    }
    \label{fig:msi_f1_per_class}
\end{figure}

==> figure/overall_system.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{figure/Overall_System.pdf}
    \caption{The proposed system for using virtual IMU data for human activities with subtle motions.
    The illustration shows six activity-class examples, where each of two classes are low, mid, and high rMSI activities. 
    (Left Upper) Virtual IMU data is extracted from Video datasets that belong to each class.
    Then, for each segmented analysis window, MSI is calculated from the corresponding original video segment source.
    The virtual IMU segments are categorized into low, mid, and high MSI samples according to the threshold values, $Th^V_L$ and $Th^V_H$, for low and high MSI values, respectively.
    (Left Bottom) From each class samples for real IMU data, the mode of rMSI per class, rMSI$_c$, is derived from the rMSI distributions in each class .
    Then, the activity classes are categorized into low, mid, and high rMSI activities according to threshold values, $Th^R_L$ and $Th^R_H$, for low and high rMSI values respectively.
    (Right) The virtual IMU data at each class is selected according to the rMSI category it belongs to.
    The selected virtual IMU data sample and real IMU data is used for model training and deployment.
    }
    \label{fig:overall_system}
\end{figure*}

==> figure/per_class_f1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/daily_activity/all_cls_f1_only_all.pdf}
    \vspace{-0.3in}
    \caption{F1 score change when using virtual IMU dataset additionally to real IMU data (20\%). 
    The baseline model only used real IMU data (20\%) for training the model.}
    \label{fig:per_class_f1}
\end{figure}

==> sections/conclusion/prev/_tmp.tex <==
\section{Conclusion}

IMUTube system was designed to capture substantial motions in underlying activities for converting human activity video into virtual IMU dataset, and was demonstrated to be extremely effective for activities with coarse movements, such as locomotion or gym exercises.
However, human activities in daily livings in fact involve much subtle motions in many context, such as eating, cooking, or washing hands that are important to assess the quality of life.
In this work, we studied the use of virtual IMU data with respect to such subtle motions in daily livings to understand the working and failing scenario of virtual IMU dataset.

To assess the utility of virtual IMU data in the context of subtle motions, we proposed a novel metric, \textit{Motion Subtlety Index} (MSI), to quantify the subtlety of motions in human activity videos that was highly correlated with actual amount of motion captured in real IMU dataset.
With MSI, we devised a system that can effectively select the segments of the video that will derive virtual IMU data with similar level of motion that reflects most probable signals captured with real IMU data.
The proposed system demonstrated that, when only sparse real IMU data is available, matching the motion subtlety of real and virtual IMU data for model training is critical to improve classification performances.

More importantly, our analysis identified the uncanny valley with respect to motion subtlety when IMUTube system miserably fails and even harms the classification performances.
IMUTube turned out to be useful when underlying human activiy involved either nearly motionless or large motions.
Any activity in between them are more likely not to benefit from IMUtube system.
We consider the major suspect of IMUTube failure is in the current limitation of 3D human motion tracking techniques, that cannot capture detailed hand and wrist coordination for subtle movements.

Overall, quantifying subtlety of the motion through MSI will provide a practical guideline to understand the degree of performance gain that can be expected from virtual IMU data in relation to particular human activities of interest, which helps for allocating time and resources for the systems like IMUTube.
Although this study takes an important step toward the application of virtual IMU data for human activities with subtle motions, it is limited to wrist motions and handful of human activities.
Therefore, our findings calls for the new research opportunity 1) to explore the use of MSI and virtual IMU data for various on-body sensor locations and wider range of human activities that involves subtle motions, and 2) to resolve the challenges in related techniques in tracking subtle motions for computer vision, graphics and biomechanics research communities.

==> sections/conclusion/prev/_tmp2.tex <==
\section{Conclusion}

In this work, we studied the use of virtual IMU data with respect to subtle motions in daily livings to understand the working and failing scenario of virtual IMU dataset. 
To quantify the subtlety of motions in human activity videos, we proposed a novel metric, \textit{Motion Subtlety Index} (MSI), and measured the subtlety of motions involved in various daily activities, which is then associated with the changes in classification performances coming from using virtual IMU dataset.
Our analysis identified the sweet spot of MSI ($0.35 \leq MSI \leq 3.33$) where adding virtual IMU data will more likely to improve the classification performance than not.

Furthermore, we analyzed how the selection of virtual IMU data according to MSI value impacted classification performance on each activity.
This revealed that activities with lower MSI preferred virtual IMU data with lower MSI values for training, and similarly for the activities with high MSIs.
Matching MSI of virtual and real IMU data could significantly improve classification performance compared to naively using all virtual IMU data available.
However, these success came with certain limitations.
Performance improvements were visible only when the activity MSI fell into the range of sweet spot, and the model started to ignore virtual IMU data as more real IMU data becomes available.
We consider the major suspect of IMUTube failure is in the current limitation of 3D human motion tracking techniques, that cannot capture detailed hand and wrist coordination for subtle movements.

Overall, quantifying subtlety of the motion through MSI will provide a practical guideline to understand the degree of performance gain that can be expected from virtual IMU data in relation to particular human activities of interest.
Knowing the falling point can help planning the resource allocation when using the systems like IMUTube for developing activity classifier.
Although this study takes an important step toward the application of virtual IMU data for human activities with subtle motions, it is limited to wrist motions and handful of human activities.
Therefore, our findings calls for the new research opportunity 1) to explore the use of MSI and virtual IMU data for various on-body sensor locations and wider range of human activities that involves subtle motions, and 2) to resolve the challenges in related techniques in tracking subtle motions for computer vision, graphics and biomechanics research communities.

==> sections/discussion/prev/_tmp.tex <==
It involves repeated hand movement to the mouth, which varies vastly depending on the eating habits and food consumed. 

The intuition comes from the mechanism of IMUTube that heavily relies on 3D motion tracking of joint keypoints observed in the scene~\cite{}.
When it comes to generating wrist sensor data, human motion tracking techniques are able to detect approximated location and motions of wrist keypoints.
This makes virtual IMU data capture wrist motions that involves arm movements, as this arm motion consists of majority of signal.
However, simply detecting and tracking wrist movements cannot tell minute wrist movements coming from hand movements or wrist rotations that involves less of arm motions.
Being this said, 

Quantifying subtlety of the motion in the video will provide a practical guideline to understand the degree of performance gain that can be expected from virtual IMU data in relation to particular human activities of interest. 

We hypothesize that MSI can be used to distinguish human activities that can be improved by using IMUTube system, which helps to prevent investing time and effort to collect virtual IMU data from videos.

\subsection{Activity-specific Effectiveness of Virtual IMU Data}
\subsubsection{Real vs. Virtual IMU data}

\subsection{Challenges in Video Quality regarding Motion Tracking}

\subsection{Quantifying the subtlety of Activity from Videos}

\subsection{Subtlety of Activity vs. Effectiveness of Virtual IMU Data}

==> sections/discussion/prev/_tmp2.tex <==
% Keeping the text from 10/02/2022

\section{Discussion}

Our experiment results demonstrated that employing MSI and using virtual IMU data with motion subtlety that corresponds to the activity class can help improve model performance when only sparse real IMU data is available.
Here, we study in-depth for the effect of MSI and real IMU data size for classifying activities with subtle motions.

\subsection{MSI vs. Classification Performance}
\label{sec:msi_f1_all}

\input{figure/msi_vs_f1}


\autoref{fig:msi_f1} explores the changes in classification performance  according to the MSI values of the virtual IMU dataset used for model training.
To effectively show the role of MSI, we used 20\% of real IMU data for each task as virtual IMU data were more useful when real IMU data was sparse.
MSI value (x-axis) was used as a upper threshold value to include virtual IMU data for model training.
For example, when MSI threshold was 7.5, all virtual IMU data with MSI below 7.5 was used for the model training.
For cut-off values, we picked 10 to 100 percentile values in entire virtual IMU dataset.
We measured the changes in F1 score (y-axis) compared to our baseline model which were trained only with real IMU dataset. 
Also, we used virtual IMU data from the curated video dataset in this analysis.

For 17 activity classes overall in daily activity classification (Left), the optimal MSI value was the 20 percentile of the entire virtualIMU dataset.
This is consistent with hypothesis that for classifying activities with subtle motions are preferred.
As MSI value has increased, the F1 score converged to the point not adding any merit for the model.

\hyeok{For Eating activity, I am waiting for the results from ZiKang}

\input{figure/msi_vs_f1_per_class}

Seeing that (\hl{hypothetically}) classification performance is significantly affected by MSI, we investigated further into how MSI values affects per-class F1 score in daily activity classification task.
We used 20\% of real IMU data similarly to the previous analysis.
\autoref{fig:msi_f1_per_class} shows four example activities for classification performance according to MSI value thresholds.
The analysis shows that the optimal MSI value depends on the activity.
Interestingly, low MSI activities (Eat with hand and Driving Automatic) preferred lower MSI values, mid MSI activities(flipping) and high MSI activities preferred higher MSI values, which alings with our hypothesis that the model benefits more when the provided virtual IMU data capture the quantity of motions reflecting the underlying activities.

\input{figure/low_mid_high_real}

\subsection{Low/Mid/High MSI Classes vs. Real IMU Scale}
\label{sec:msi_group_real_size}

Observing that the optimal MSI values are very specific to subtlety of motions of the involved activity, we hypothesized that the impact of virtual IMU data will increase even in the presence of large real IMU dataset, if activities with similar motion levels are classified together with virtual IMU data also having similar level of motions.
To validate this hypothesis, we explored the classification performance when classification is performed only within the groups of low, mid, and high MSI activities.
Also,we changed the amount of real IMU data for model training at the same time.
We independently trained low, mid, high MSI activity groups with virtual IMU data with low, mid, high MSI values, respectively.
For each case, we also compared the classification performance when using all virtual IMU dataset.

\autoref{fig:low_mid_high_real} demonstrates F1 score for each cases also including when using all activity classes combined with the proposed method.
When classifying with only low-MSI activities (left upper), the low-MSI virtual IMU data was especially effective $7+$ F1 score increase even when the 50\% of real IMU data was used.
When there is little to no motion, It is feasible for IMUTube to capture such activities reliably.
Intuitively speaking, those activities will be reflected in almost no movements in 3D motion tracking information that is transferred to virtual IMU dataset.
For high MSI activity classification (left bottom), only using high-MSI virtual IMU data significantly outperformed naively using all virtual IMU data for model training for all cases.
This reflects that choosing appropriate virtual IMU data through MSI is important, but with the limited success.
As soon as more than 30\% of real IMU was used, the effect of virtual IMU data was negligible.
Even for high MSI activities here, they are still in the domain of \textit{subtle motions}, which is difficult to track with state-of-the-art 3D motion tracking pipeline that roughly estimated joint locations.

For mid MSI activity classification (right upper), the effect of virtual IMU data was trivial or even degrading the model performance even when using MSI.
This exactly demonstrates the breakdown points of IMUTube system.
When the activity is nearly motionless but has still very subtle motions at the same time in the point of motion tracking view, it is the uncanny valley where IMUTube system completely fails to capture quality virtual IMU dataset.
All activities combined (right bottom), the proposed method could benefit from virtual IMU data with MSI only up to 40\% of real IMU dataset.
We suspect the inclusion of mid-MSI motions have suppressed the gain from either low or high MSI motions.

Overall, this study demonstrates the working and failing scenario of IMUTube.
IMUTube either prefers the activity is nearly motionless or with larger motions, which closely follows current limitation of state-of-the-art human motion tracking techniques~\cite{desmarais2021review}.
When the motion quantity of underlying activity falls into somewhere in between, then IMUTube is likely to fall out.
Our study shows usefulness of the proposed MSI, which can tell if an activity of interest falls into this uncanny valley for IMUTube or not.










==> sections/discussion/prev/_tmp3.tex <==
%text keep 10/05/2022

\section{Discussion}

\hyeok{Need to update all analysis with the results when using all real IMU data.}

The earlier experiment results demonstrated that the utility of virtual IMU to heavily depend on the amount of motion involved in activity classes.
Virtual IMU data was very effective when capturing various arm motions in eating activities, whereas it was having difficulty capturing subtle hand and wrist motions in other daily activities.
In this section, we further investigate the relationship between the motion subtlety in activities and classification performance through our proposed MSI.

\subsection{MSI vs. Classification Performance}
\label{sec:msi_f1_all}

\input{figure/per_class_f1_real_100}
\input{figure/msi_f1_spline}

To understand for which activity virtual IMU data was most useful, \autoref{fig:per_class_f1} shows the detailed classification performance changes for each class in daily activity classification task by adding virtual IMU dataset for model training.
The baseline model is trained with 20\% of real IMU data.
Performance change had a wide range of variability ($\pm 10$ absolute F1-score).
Performance gain was significant (absolute 5+\%) for activities like wiping, washing hands, reading, flipping, playing guitar.
Whereas significant loss (absolute 5-\%) was observed for drawing, writing, playing violin, and cutting activities.

We studied the relationship between the MSI score for each activity with the changes in F1 score.
\autoref{fig:msi_f1_spline} shows the spline curve fitting on the data points for the MSI mode and the corresponding F1 score changes of each class introduced by using virtual IMU data.
As representative MSIs for each activity, we picked mode MSI from the distribution of MSI for each class.
This analysis shows that there exists a range of MSI values ($0.35 \leq MSI \leq 3.33$) that are more likely to increase the model performance (2.5+\%, \textcolor{red}{red line}) by using virtual IMU dataset.
Extremely low subtlety of motions ($MSI < 0.35$) such as drawing or writing were very difficult for IMUTube to extract useful virtual IMU data, and the mid range ($3.33 < MSI < 7.46$) or high range ($7.46 < MSI$) MSI activities showed mixed results but with overall expectation with only marginal or negative impact on model performance when using virtual IMU dataset.
To much of our surprise, this finding suggested that there exists a sweet spot of MSI that can still make IMUTube useful even for the activities with subtle motions.

\subsection{MSI for Virtual IMU Data Selection}

\input{figure/msi_vs_f1}
We further assess the how does the class-specific classification performance varies according to MSI value used in daily activity classification task.
\autoref{fig:msi_f1} explores the changes in classification performance  according to the MSI values of the virtual IMU dataset used for model training.
To effectively show the role of MSI, we used 20\% of real IMU data for each task as virtual IMU data were more useful when real IMU data was sparse.
MSI value (x-axis) was used as a upper threshold value to include virtual IMU data for model training.
For example, when MSI threshold was 7.5, all virtual IMU data with MSI below 7.5 was used for the model training.
For cut-off values, we picked 10 to 100 percentile values in entire virtual IMU dataset.
We measured the changes in F1 score (y-axis) compared to our baseline model which were trained only with real IMU dataset. 
Also, we used virtual IMU data from the curated video dataset in this analysis.

For 17 activity classes overall in daily activity classification (Left), the optimal MSI value was in the range of $0.35 \leq MSI \leq 3.33$, which was consistent with the earlier annalysis.
As MSI value has increased, the F1 score converged to the point not adding any merit for the model.

\hyeok{For Eating activity, I am waiting for the results from ZiKang}

\input{figure/msi_vs_f1_per_class}

Seeing that classification performance is significantly affected by MSI, we investigated further into how MSI values affects per-class F1 score in daily activity classification task.
We used 20\% of real IMU data similarly to the previous analysis.
\autoref{fig:msi_f1_per_class} shows four example activities for classification performance according to MSI value thresholds.
The analysis shows that the optimal MSI value depends on the kind of activity.
Interestingly, low MSI activities (Eat with hand and Driving Automatic) preferred lower MSI threshold values, mid (flipping) and high MSI activities preferred higher MSI threshold values to improve classification performance.
This may indicate that the model benefits more when the provided virtual IMU data capture the quantity of motions reflecting the underlying activities.

\subsection{Low/Mid/High MSI Classes vs. Real IMU Scale}
\label{sec:msi_group_real_size}

Observing that the optimal MSI values for each activity are very specific to subtlety of motions of involved activity, we hypothesized that the impact of virtual IMU data will increase, if virtual IMU data provided for each activity had similar level of motion subtlety as in the corresponding target activity. 
To validate this hypothesis, we categorized each activity in to low, mid, and high MSI groups according to mode MSI values of each activity.
The low MSI group included reading, driving automatic, drawing, eating, playing guitar, the mid MSI group included playing violin, writing, driving manual, flipping, playing piano, cutting components, wiping, and the high MSI group included bed making, shower, sweeping, washing hands, washing dishes.

For activities in each MSI group, we assigned virtual IMU data with the similar amount of motion subtlety according to the MSI values.
Virtual IMU data from all classes are categorized into low, mid, and high MSI groups ($MSI_{low} < 3$, $3 \leq MSI_{mid} <6$, and $6 \leq MSI_{high}$) according to our observation in \autoref{fig:msi_f1_spline}.
For model training, we only used virtual IMU data with $MSI_{low}$ for low MSI group activities, $MSI_{mid}$ for mid MSI group activities, and $MSI_{high}$ for high MSI group activities.

\input{figure/low_mid_high_real}

\autoref{fig:low_mid_high_real} shows the effect of matching motion subtlety between real and virtual IMU data for model training.
We independently trained low (upper left), mid (upper right), high (bottom left) MSI activity groups, and also, trained for all activity classes combined (bottom right).
For each case, we also compared the classification performance when naively using all virtual IMU dataset.
We additionally changed the amount of real IMU data for model training (x-axis) to better understand the impact of real IMU dataset.

When classifying with only low-MSI activities (left upper), the low-MSI virtual IMU data was especially effective $7+$ F1 score increase even when the 50\% of real IMU data was used.
Consistent with previous analysis, this range of motion subtlety was most effective region for IMUTube.
For mid MSI activity classification (right upper), the effect of virtual IMU data was trivial or even degrading the model performance even when using MSI.
This exactly demonstrates the breakdown points of IMUTube system.

For high MSI activity classification (left bottom), only using high-MSI virtual IMU data significantly outperformed naively using all virtual IMU data for model training for all cases.
This reflects that choosing appropriate virtual IMU data through MSI is important, but with the limited success.
As soon as more than 30\% of real IMU was used, the effect of virtual IMU data was negligible.
Although they fall into high MSI groups in our analysis, they are still the activities with \textit{subtle motions}, which is difficult to track with state-of-the-art 3D motion tracking pipeline that roughly estimated joint locations.
All activities combined (right bottom), the proposed method could benefit from virtual IMU data with MSI only up to 40\% of real IMU dataset.
We suspect the inclusion of mid-MSI motions have suppressed the gain from either low or high MSI motions.

Overall, this study demonstrates the working and failing scenario of IMUTube when it comes to subtle activities.
Activity classes beyond $3\leq MSI$ seems to have subtle yet very complex motions in hand and wrist movements that are very difficult for IMUTube to capture, which closely follows current limitation of state-of-the-art human motion tracking techniques~\cite{desmarais2021review}. 
Also, as more real IMU data become available, the model starts to ignore virtual IMU data. 
Therefore, amount of real IMU data is another important factor to consider when choosing to use IMUTube for subtle activities.












==> sections/experiment/prev/_tmp.tex <==
%----------------------------------
% For keeping the text
%----------------------------------

\subsection{IMUTube with MSI}

\input{tables/dataset}

\thomas{Coming back to my thoughts on the introduction: Why don't we lead with the analysis of subtlety of the movements underlying activities of daily living? That would make one fine, strong contribution on its own and put the experiments (and the findings!) on a solid foundation. Thoughts?}

Evaluating IMUTube requires benchmarking different datasets that cover a variety of \textbf{fine motion} \thomas{fine or subtle?} activities along with video datasets that can be used to extract the required virtual IMU data. 
We mainly studied classification tasks on two sets of representative activities with fine motions using wrist sensors: 1) Eating~\cite{thomaz2015practical}, and 2) daily activities~\cite{inproceedings}.



In what follows, we discuss benchmark datasets and virtual IMU data used to analyze the effectiveness IMUTube on such subtle motions in activities.
\autoref{tab:dataset} shows statistics of the dataset used in our experiments.
\thomas{See my comment above re leading with the index. Also: This is too eating-centric again, no?}

\thomas{We should also fork out the details of the overall processing pipeline, which is not data related. So, have a separate subsection on the classification backend, training procedure, IMUTube configuration (calibration and such). We need to provide as much detail here as we can, such that the results can be interpreted well (and be trusted!).}

\thomas{I am also missing some sort of an overview on the experiment protocol: What do we do with the individual datasets? How do we feed them into the IMUTube system? Any parameter optimization? How do we measure effectiveness? We can cover all this in one leading, separate subsection where we describe all details independent of the actual datasets -- that comes later, and can then be much more streamlined and compressed. We could have a workflow figure here that illustrates the overall procedure. We do have the space.}

\subsection{Eating Recognition}

\input{figure/eating}

\subsubsection{Benchmark Real IMU Dataset}

For eating detection, we used a large public dataset from Thomaz~\etal~\cite{thomaz2015practical} that contains both in-lab and in-the-wild real IMU data for benchmarking IMUTube.
This choice was motivated by previous work \cite{thomaz2015practical,bedri2015wearable, bedri2017earbit, bedri2020fitbyte}, which focused on develop eating moment recognition solutions in controlled settings that can also work well in-the-wild.
The \textit{Lab-20} dataset was collected from 21 participants between the ages of 20 and 43 covering both eating and non-eating activities for approximately 31 minutes period on average. 
The activities contained a mix of eating and non-eating moments with no time constraints on participants. The eating moments involve,
eating with fork \& knife, 
hand, 
and spoon
while non-eating activities include 
watching trailer, conversation,
brush teeth,
place a phone call etc., all being \textit{fine hand} motions. 
For in-the-wild experiments, we used the \textit{Wild-7} dataset \cite{thomaz2015practical}, which was collected from seven participants between the ages of 21 and 29 throughout the day using wrist sensors and wearable cameras. 
Out of a total of 31 hours and 28 minutes of data, 2 hours and 8 minutes were labeled as eating activities.
Similar to previous work \cite{thomaz2015practical}, we applied a DBSCAN \cite{ester1996density} based analysis approach to determine eating moments.
\thomas{Given that we only use that dataset, we may want to compress this presentation here a bit.}

\subsubsection{Curated Video Dataset}

For assessing the feasibility, we first collected virtual IMU data from well curated video dataset, Kinetics-400 \cite{kay2017kinetics}, where all videos were manually trimmed down to clips of  10 seconds to contain specific activity classes. 
In our experiments, we used 417 video clips for the eating class, which were labeled as one of 10 eating-related classes (eating: burger, cake, carrots, chips, doughnuts, hotdog, ice cream, nachos, spaghetti, watermelon). 
The extracted virtual IMU data contained approximately 6\% more eating instances compared to Lab-20 dataset.

\subsubsection{In-the-wild Video Dataset}

YouTube houses one of the largest collection of uncurated videos that are coarsely labeled using Google's search algorithm, providing a virtually unlimited source of videos for any activity. 
We download two YouTube videos that were labeled as "eating" (through our search query and brief thumbnail inspection for the returned results):
The first video is 22 minutes long, whereas the second one has a duration of 17 minutes.
As shown in \autoref{fig:eating}, videos from online repositories contain scenes that do not involve human eating motions, i.e., scenes that IMUTube~\cite{kwon2021approaching} can automatically filter out with Adaptive Video Selection modules (yellow box;\autoref{fig:imutube}).
However, we could already collect 11\% more eating data samples compared to eating instances in Lab-20 dataset from those two videos combined.

\subsubsection{Experiment Protocol}

For our eating detection experiment, we use Lab-20 dataset as training set and Wild-7 as testing set.
Our baseline model is trained only with real IMU data from Lab-20 dataset.
Our proposed model is trained with both real and virtual IMU dataset, where virtual IMU dataset is either from curated or in-the-wild video dataset.
the collected virtual IMU dataset is weakly labeled as search keyword 'eating' was used for labels.
Following the standard process in IMUTube~\cite{kwon2020imutube}, virtual IMU data was calibrated with training real IMU data from the lab (Lab-20) for model training.

For model training and evaluation, we sub-sampled the real IMU data to 25 Hz to match the sampling rate of the virtual IMU dataset extracted from videos.
Following previous eating studies \cite{thomaz2015practical}, we applied sliding window segmentation with 6 second window size and 50\% overlap between consecutive analysis frames, and extracted mean, variance, skewness, kurtosis and root mean square features from each frame.
The choice of window length was kept such that the whole eating activity could be completed within this time window
We trained Random Forest (RF) model and reported binary F1-scores from the average of three runs on on Wild-7 dataset.
\thomas{See my comment above on a separate subsection that covers the recognition backend detals.}

\subsection{Recognition of Daily Activities with Subtle Motions}

\subsubsection{Benchmark Real IMU Dataset}
Many daily activities include far more subtle motions compared to eating activities.
To further test IMUTube systems on such fine activities, we used HAD-AW dataset \cite{inproceedings} as our benchmark dataset, which consists of 31 activity classes, including bed-making, flipping pancakes, and showering, in total that is collected from a smart watch.
The volunteers' age ranges from 25 to 55 years old, weights from 55 kg to 95 kg and have representation from both males and females. The data is collected using an Apple Watch worn by the candidates and have 160 samples on average per activity. 
Not all of 31 activity classes are fine activities.
Thus, we selected 17 activity classes for our experiments:
playing violin,
playing piano,
playing guitar,
driving automatic,
driving manual,
reading,
writing,
eating,
cutting components,
washing dishes,
washing hands,
showering,
sweeping,
wiping,
drawing,
flipping,
bed-making.

\subsubsection{Curated Video Dataset}

\input{figure/daily_activity}

For the feasibility test, we collected well curated video dataset from Kinetics-400 dataset for 17 activity classes used for experiments.
In total, we collected virtual IMU dataset with approximately 50\% of the size of real IMU dataset from HAD-AW dataset.
As shown in \autoref{fig:daily_activity_data_proportion}, the virtual IMU samples are imbalanced due to many video clips posing challenges to extract virtual IMU for wrist movements.
IMUTube system automatically filters the scenes that are challenging for effective motion tracking, which has risk of collecting low-quality virtual IMU data, such as scenes including zoomed-in focus on hand movements not showing entire arm movements or occlusions on wrist motions due to viewing angles.

\subsubsection{In-the-wild YouTube Video Dataset}

\hyeok{TK-Waiting for Zikang to get the data and results.}

\subsubsection{Experiment Protocol}

For the experiment with HAD-AW dataset, the real IMU datasets were downsampled to 25 Hz to match the sampling rate with virtual IMU datasets from videos.
We applied 5-fold stratified cross-validation.
we could not test leave-one-user-out cross validation, as some activities were only performed by a single user.
All real and virtual IMU data were segmented with sliding window of 3-second analysis frames with step size of 1.5-second following the previous work~\cite{inproceedings}.
We extracted ECDF features~\cite{hammerla2013preserving} from each analysis frame.
Our baseline model was the model trained only with real IMU dataset, and proposed model was the model trained with both real and virtual IMU datasets.
We used Random forest model for all experiments and reported mean F1 score average from three runs from all cases.
When we use virtual IMU dataset, we calibrated virtual IMU dataset with the training real IMU data at each fold likewise the standard protocol used in IMUTube.


==> sections/experiment/prev/_tmp2.tex <==
% keeping text 10/02/2022
\section{Experiment}
\thomas{See my other comment. I am very confused why the entire logic has been put upside down now.}
In our experiments, we will analyze the effectiveness of MSI for quantifying the subtlety of movements in various daily activities through conduct correlation study between MSI and rMSI. \thomas{No! rMSI has no proven relevance for any practical outcome. At the end of the day, it is the F1 scores on HAR tasks that matter.}
Then, we compare recognition performance for daily activity classification tasks using virtual IMU data  MSI and rMSI with and without.
Here, we introduce our experiment settings and the benchmark datasets used for annalysis.

\subsection{Classification with Virtual IMU Data, MSI, and rMSI}

We followed the approach used in the original IMUTube experiments \cite{kwon2020imutube}.
We extracted virtual IMU data for wrist sensors from video datasets, which are calibrated with (the small amounts of) real IMU data used for training.
Real IMU data is subsampled to 25 Hz to match the sampling rate of virtual IMU data from videos.
Both virtual and real IMU data are segmented into analysis frames, for example 4-seconds window, using sliding window operation.
The choice of window size depends on the particular activity of interest
For calculating MSI, we segment video sequence where each virtual IMU analysis frame is originated from.
Then, optical flow~\cite{farneback2003two} and 2D pose~\cite{fang2017rmpe} is estimated from video segments, which are used to calculate MSI for each virtual IMU analysis frame.
rMSI is directly calculated from the segmented real IMU analysis frames.
Based on the calculated rMSI and MSI, the virtual IMU analysis frames are selected for model training according to low/mid/high motion subtlety for involved activity classes.
Then, reatures are extracted from both real and virtual analysis windows, which is used to train a classification backend model, where we use Random Forest in this study.
Lastly, the trained model is then tested on unseen real IMU dataset.

Our baseline models are 1) the model trained only with real IMU data and 2) the model trained with both real and virtual IMU dataset.
Our proposed model additionally uses MSI and rMSI when trained with both real and virtual IMU dataset.
Virtual IMU datasets are either from curated or in-the-wild video dataset as explained below.

\input{tables/dataset}

\subsection{Benchmark Real IMU Dataset}

In this work, we do not consider activities with inherently coarse movements, such as locomotion or exercises, that involves nearly full-body motion signals, which is already well-studied in the previous work~\cite{kwon2020imutube,kwon2021approaching}.
For studying subtle motions in daily activities, we use two benchmark datasets for wrist sensors: daily activity classification~\cite{inproceedings} and eating activity classification~\cite{thomaz2015practical}.
\autoref{tab:dataset} shows statistics of the dataset used in our experiments.

\subsubsection{Daily Activity}

We used HAD-AW dataset \cite{inproceedings} as our benchmark dataset, which consists of 31 activity classes from subtle to coarse motions collected using an Apple Watch. 
Out of all of 31 activity classes, we selected 17 activity classes with subtle motions for our experiments:
playing violin,
playing piano,
playing guitar,
driving automatic,
driving manual,
reading,
writing,
eating,
cutting components,
washing dishes,
washing hands,
showering,
sweeping,
wiping,
drawing,
flipping,
bed-making.

\subsubsection{Eating Activity}

We used a large public dataset from Thomaz~\etal~\cite{thomaz2015practical} that contains both in-lab and in-the-wild real IMU data for benchmarking IMUTube.
The \textit{Lab-20} dataset was collected from 21 participants in the lab covering both eating and non-eating activities for approximately 31 minutes period on average. 
The eating moments involve,
eating with fork \& knife, 
hand, 
and spoon.
While non-eating activities include 
watching trailer, conversation,
brush teeth,
place a phone call etc., all being subtle hand motions. 
For in-the-wild datset, we used the \textit{Wild-7} dataset \cite{thomaz2015practical}, which was collected from seven participants. 
Out of a total of 31 hours and 28 minutes of data, 2 hours and 8 minutes were labeled as eating activities.
% \thomas{Given that we only use that dataset, we may want to compress this presentation here a bit.}

\subsection{Curated Video Dataset}

For assessing the feasibility for using virtual IMU data for subtle motions, we first collected virtual IMU data from well curated video dataset, Kinetics-400 \cite{kay2017kinetics}, where all videos were manually trimmed down to clips of 10 seconds to contain specific activity classes. 

\subsubsection{Daily Activity}

\input{figure/daily_activity}

We collected well curated video dataset from Kinetics-400 dataset for 17 activity classes used for experiments.
In total, we collected virtual IMU dataset with approximately 50\% of the size of real IMU dataset from real IMU dataset.
As shown in \autoref{fig:daily_activity_data_proportion}, the virtual IMU samples are imbalanced, as many video clips are removed due to the challenging scenes for extracting virtual IMU for wrist movement.

\subsubsection{Eating Activity}

We used 417 video clips for the eating class, which were labeled as one of 10 eating-related classes (eating: burger, cake, carrots, chips, doughnuts, hotdog, ice cream, nachos, spaghetti, watermelon). 
The extracted virtual IMU data contained approximately 6\% more eating instances compared to Lab-20 dataset.

\subsection{In-the-wild Video Dataset}

YouTube houses one of the largest collection of uncurated videos that are coarsely labeled using Google's search algorithm, providing a virtually unlimited source of videos for any activity. 
As shown in \autoref{fig:eating}, videos from online repositories contain scenes that do not involve human eating motions, i.e., scenes that IMUTube~\cite{kwon2021approaching} can automatically filter out with Adaptive Video Selection modules (yellow box;\autoref{fig:imutube}).
We downloaded videos from YouTube using activity class as search keywords, where queried videos are sorted according to relevance.

\subsubsection{Daily Activity}

We downloaded one video for each class, which were approximately 8 minutes of video clips on average per activity.
We could collect approximately 16\% size of virtual IMU data compared to real IMU benchmark dataset.
% \hyeok{TK-Waiting for Zikang to get the data and results.}

\subsubsection{Eating Activity}

We download two YouTube videos, where the first video is 22 minutes long, and the second one has a duration of 17 minutes.
From those two videos combined, we could collect 11\% more eating data samples compared to eating instances in Lab-20 dataset.

\input{figure/eating}

\subsection{Hyperparameters}

Here we explain specific settings and hyperparmeters we used for dailty activity and eating recognition tasks.

\subsubsection{Daily Activity}

We applied 5-fold stratified cross-validation.
we could not test leave-one-user-out cross validation, as some activities were only performed by a single user.
All real and virtual IMU data were segmented with sliding window of 3-second analysis frames with step size of 1.5-second following the previous work~\cite{inproceedings}.
We extracted ECDF features~\cite{hammerla2013preserving} from each analysis frame.
Threshold values when using MSI and rMSI were $TH^V_L=3$, $TH^V_H=6$, $TH^R_L=0.05$, and $TH^R_H=0.1$.
Among 17 classes, the low MSI group included reading, driving automatic, drawing, eating, playing guitar, the mid MSI group included playing violin, writing, driving manual, flipping, playing piano, cutting components, wiping, and the high MSI group included bed making, shower, sweeping, washing hands, washing dishes.
We reported mean F1 score average from three runs from all cases.

\subsubsection{Eating Activity}

We use Lab-20 dataset as training set and Wild-7 as testing set.
Accordingly, virtual IMU data was calibrated with Lab-20 dataset.
Following previous eating studies \cite{thomaz2015practical}, we applied sliding window segmentation with 6 second window size and 50\% overlap between consecutive analysis frames, and extracted mean, variance, skewness, kurtosis and root mean square features from each frame.
The predictions from the trained Random Forest (RF) model was applied with DBSCAN clustering to determine eating moments with the best hyperparameter from previous work \cite{thomaz2015practical}, where a minimum number of intake gestures is two (minPts=2) and a distance measure given as a temporal neighborhood was 80 (eps=80).
Threshold values when using MSI and rMSI were $TH^V=4.5$ and $TH^R=0.06$.
We reported binary F1-scores from the average of three runs on on Wild-7 dataset.
% \thomas{See my comment above on a separate subsection that covers the recognition backend detals.}

% \thomas{Coming back to my thoughts on the introduction: Why don't we lead with the analysis of subtlety of the movements underlying activities of daily living? That would make one fine, strong contribution on its own and put the experiments (and the findings!) on a solid foundation. Thoughts?}\hyeok{Yes. We will do that in the Result section. This section is only to introduce experiment protocols and datasets used to discuss our results.}
% \thomas{See my comment above re leading with the index. Also: This is too eating-centric again, no?}
% \thomas{We should also fork out the details of the overall processing pipeline, which is not data related. So, have a separate subsection on the classification backend, training procedure, IMUTube configuration (calibration and such). We need to provide as much detail here as we can, such that the results can be interpreted well (and be trusted!).}
% \thomas{I am also missing some sort of an overview on the experiment protocol: What do we do with the individual datasets? How do we feed them into the IMUTube system? Any parameter optimization? How do we measure effectiveness? We can cover all this in one leading, separate subsection where we describe all details independent of the actual datasets -- that comes later, and can then be much more streamlined and compressed. We could have a workflow figure here that illustrates the overall procedure. We do have the space.}\hyeok{The workflow figure is introduced in the method section.}

==> sections/method/prev/_tmp.tex <==
Subtlety of motion differs according to the underlying human activity of daily living, and we consider wrist motions can be categorized into \textit{stationary}, \textit{hand}, or \textit{arm} motion activities.
\textit{Stationary} (or still) motion is when majority of human motion involved in underlying activity is stationary majority of the time, such as reading or driving activities.
\textit{hand} motion category is when subtle movements are coming from hand or finger motions with minimum involvement of arm motions, such as drawing or playing guitar.
\textit{arm} motion is when the motion involves entire arm movements such as 
repetitive motions periodically over the span of activity, such as eating with silver wares.
In this work, we do not consider activities with inherently coarse movements, such as locomotion or exercises, that involves nearly full-body motion signals, which is already well-studied in the previous work~\cite{kwon2020imutube,kwon2021approaching}.

We consider that IMUTube would generate useful virtual IMU data when the motion is either \textit{stationary} or \textit{repetitive} with respect to the on-body sensor location, but the system miserably breaks down when it were to capture more \textit{sporadic} activities with subtle movements with providing no gain or even harming the model trained with virtual IMU data.
The intuition comes from the mechanism of IMUTube that heavily relies on 3D motion tracking of joint keypoints observed in the scene~\cite{}.
When it comes to generating wrist sensor data, human motion tracking techniques are able to detect approximated location and motions of wrist keypoints.
This makes virtual IMU data capture wrist motions that involves arm movements, as this arm motion consists of majority of signal.
However, simply detecting and tracking wrist movements cannot tell minute wrist movements coming from hand movements or wrist rotations that involves less of arm motions.
Being this said, 

==> sections/method/prev/_tmp2.tex <==
% Keeping text for 10/02/2022
\section{Method}

\subsection{Quantifying Motion Subtlety in Human Activity}

The IMUTube system was originally designed to capture substantial body (part) movements in human activity videos -- information, which is subsequently transferred to \textit{virtual} IMU data.
In this work, we aim to study how such system can be used when studying human activities with only \textit{subtle} underlying movements.
Essentially, we aim to explore what the ``breaking point'' of IMUTube-like approaches us, i.e., what the limits of its applicability--beyond the originally studied coarse movement activities--are.
We define subtle motions in human activities as those movements that involve one or two body parts moving in the very limited range of distances.
For example, activities such as  washing hands, writing, cooking, eating, and so on, involve only hand or arm movements that are much smaller in range compared to activities that are based on whole-body involvement, such as sports or gym exercises.

\input{figure/motion_subtlety}

\subsubsection{Motion Subtlety in Virtual IMU Data}
\thomas{Hold on, folks. Aren't we measuring the MSI on video data? So, why is the focus here on virtual IMU data?}
To objectively define the amount of motion subtlety in virtual IMU data, we propose \textit{Motion Subtlety Index} (MSI).
We measure motion subtlety of virtual IMU data from original source video dataset.
Specifically for human motion in the scene, 2D pose estimation is widely used to capture how much joint keypoints moved between subsequent frames~\cite{dubey2022comprehensive}.
However, pose estimation is limited in quantifying very detailed pixel-level motions, as 2d keypoints are only approximated locations of human joint locations.
This applies similarly to the virtual IMU dataset, as virtual IMU data is derived from pose estimation method so that quantifying motion subtlety from virtual IMU data directly is not sufficient for pixel-level motion subtlety.
On the other hand, conventional approaches to measure the any detailed movements in a video sequence is through the use of optical flow~\cite{zhai2021optical}.
Optical flow measures the displacement of pixels between subsequent frames, which tells the amount of motion in the local regions in each frame.
Therefore, we combine optical flow and 2D pose estimation from video sequence to quantify the pixel-level motion quantity, Motion Subtlety index (MSI) in other words.
\thomas{See my comment above: This should be about videos! Our motivation is to have some quantification that allows us to estimate the value virtual IMU data may have for HAR down the line BEFORE we do all the virtual IMU data extraction and the HAR modeling. In the language we used earlier on: we want to quantify the subtlety of human movements in videos and correlate it to the effectiveness of IMUTube-based HAR systems. So, this paragraph needs to be revised please and be made more clear. (next are fine) }

\autoref{fig:msi} illustrates how the MSI is calculated for an exemplary video that captures a sequence of writing activity with the wrist as the target location for the virtial IMU sensor. 
For each of the sequence of $T$ video frames, we first compute the optical flow and estimate 2D poses.
%estimation model from the sequence of $T$ frames of human activity RGB sequence.
Next, we calculate the average magnitude (over the entire sequence) of optical flow at the local patch, $5\times 5$, in the neighborhood of the wrist keypoint location, which is automatically detected by our 2D pose estimation procedure:
\begin{equation}
    MSI_t = \frac{1}{N} \sum_{-2\geq i,j \geq 2}  \sqrt{(v_{k + i})^2 + (u_{k + j})^2},
\end{equation}
where $v$ and $u$ are vertical and horizontal optical flow measurements from keypoint location, $(v_k, u_k)$, and $N=5 \times 5 = 25$ at time $t$.
The MSI for the analysis window is then computed as the standard deviation of $MSI_t$ across all analysis frames:
\begin{equation}
    MSI = std([MSI_1, MSI_2, \cdots, MSI_T])
\end{equation}

MSI captures the amount of motion information recorded around the on-body sensor location for underlying activities in the given video sequence.
A smaller MSI means more subtle motions are involved with on-going activities, whereas a larger MSI indicates more coarse movements.

\input{figure/overall_system}

\subsubsection{Motion Subtlety in Real IMU Data}

When it comes to quantifying subtlety of motions in real IMU dataset, we can directly compute \textit{real Motion Subtlety Index} (rMSI) from captured signals.
Given a sequence of accelerometry signal in the analysis frame, $X^{T\times 3}$, where $T$ is the duration of real IMU data, we first remove the gravity component, $\hat{X}_t = X_t - X_g$, which is the average of accelerometry signal, $X_g = \frac{1}{T}\sum_{0 \leq t \leq T} X_t$.
Then, the magnitude of acceleration is computed, $\bar{X}_t = \sqrt{\hat{x}^2_t + \hat{y}^2_t + \hat{z}^2_t}$, where $\hat{X}_t = [\hat{x}, \hat{y}, \hat{z}]$.
Lastly, rMSI is defined as the standard deviation of the magnitude of accelerometry signal without gravity components, $rMSI = std([\bar{X}_1, \bar{X}_2, \cdots, \bar{X}_T])$.
Overall, high rMSI value indicates larger motions involved for performing the on-going activity.
\thomas{I do not understand why we need the MSI on IMU?}

\subsection{IMUTube with Subtle Motions}


We hypothesize that activities with subtle motions can be further categorized into more, mildly, or less subtle activities, and that virtual IMU data is most useful when it is extracted from video sequence performing similar level of subtle motion as in target activity. \thomas{Where does that come from? I don't think it makes much sense. All we set out to is to quantify the subtlety and, then, to correlate that quantitative measure to eventual HAR accuracy outcomes. So, this sort of speculation here is, imho, not helpful, if not hurting.}
The proposed method is aimed to match the subtlety of motion captured in virtual and real IMU data for the model training so that potentially irrelevant virtual IMU data for particular activity class is avoided for using. \thomas{First time I hear about this ... Does not make much sense to me.}

Given activity classes of interest, each activity are categorized into three different amount (low, mid, high) of motions involved in performing activities.
Once rMSI is computed for all the analysis frames for real IMU data, the mode of rMSI per class, rMSI$_c$, is derived from the distribution of rMSI for each class to represent motion subtlety for each class.
Then, each class is categorized to low, mid, and high rMSI values using the threshold values, $Th^R_L$ and $TH^R_H$, for low and high rMSI, respectively.
We empirically selected $Th^R_L$ and $TH^R_H$ as 33 and 66 percentiles of the collection of rMSI$_c$ from all classes.
low, mid, and high rMSI classes are determined through $rMSI_c < Th^R_L$, $Th^R_L \leq rMSI_c \leq Th^R_H$, and $Th^R_H < rMSI_c$, respectively.
We also categorize low, mid, and high MSI for virtual IMU dataset.
From the collection of MSIs, $MSI^i$, from all virtual IMU data frames, we also select 33 and 66 percentiles, $Th^V_L$ and $Th^V_H$, as cut-off values to distinguish low, mid, and high MSI.
low, mid, and high MSI windows are determined through $MSI^i < Th^V_L$, $Th^V_L \leq MSI^i \leq Th^V_H$, and $Th^V_H < MSI^i$, respectively.

Now that we have categorized virtual IMU analysis frames that belong to low, mid, and high MSI, and categorized activity classes that belongs to low, mid, and high rMSI$_c$, we use this categorization for training the activity recognition model.
Specifically, for each class, we only use virtual IMU data that belongs to same category of motion subtlety as the activity class.
For example, if an activity class is categorized as low rMSI$_c$, then we only use virtual IMU data sample of the same class that is categorized as low MSI.
This is done similarly for other activities that is categorized as mid and high motion subtlety.
The illustration of entire process is shown in \autoref{fig:overall_system}.

For the case with binary classification, we use similar approach but with low and high categorization of the two activities and virtual IMU analysis window.
For low and high activity class, single threshold value for rMSI$_c$ and MSI, $Th^R$ for and $Th^V$, respectively.
$Th^R$ is median of two rMSI$_c$ to put each class into either low or high motion classes.
$Th^V$ is median of all MSI samples from both classes to categorize each virtual IMU analysis frame into either low or high motion classes.

\thomas{Sorry, but I do not understand the purpose of this entire section B. What we had in mind was to come up with a quantitative measure for the subtlety of movements belonging to activities -- to be calculated on videos. With that measure, we do have a characterization of a task (activity recognition) in the video domain. We then go ahead and translate a bunch of activity videos into virtual IMU data -- using IMUTube -- and train downstream HAR classifiers as we did before. We then get F1 scores for all those recognition tasks (so, look at class-specific F1 scores) and are now--post mortem--able to correlate those F1 scores back to the MSI scores (again, computed on videos). Our analysis can then tell us: for which activities does IMUTube still work. More systematically: Up to what threshold of MSI (on videos!) can we expect IMUTube to still work. So, for future application cases one would go ahead and calculate MSI values on a bunch of videos BEFORE even doing the whole IMUTube application -- which is quite a bit of effort. As such, we will be able to provide guidance on when to use IMUTube -- and when not -- through the systematic analysis of MSI as evidenced through the experiments in this paper that correlate MSI (on video) to downstream F1 scores on actual HAR experiments that were run using virtual IMU data as generated by IMUTube. So, our original goal is still to look for when IMUTube breaks but now with the additional underlying systematic approach of actually measuring the subtlety!}


==> sections/related_work/prev/_eating.tex <==
%--------------------
% Just for the sake of keeping texts for future use ...
%--------------------

\subsection{Eating Detection}

One of the primary examples of fine motion activity is eating~\cite{thomaz2015practical,bedri2017earbit,bedri2020fitbyte,bedri2015wearable}. 
It involves repeated hand movement to the mouth, which varies vastly depending on the eating habits and food consumed. 
There are also lots of similar movements in daily living that can create false positives for such detection methods.


\thomas{Trying not run in circles here, but: Why do we have a full section solely dedicated to eating detection? I thought we wanted to be broader? Has our focus been changed back to eating again?}
Amongst many daily activities, detecting eating activity has gained much interest in wearable-based human activity recognition community for its direct connection with severe health conditions, such as depression, anxiety, or obesity~\cite{konttinen2019depression,navarro2021effects,van2018causes}.
Eating detection is a mature field and many studies have been conducted in which a range of wrist based sensing and analysis systems have been utilized \cite{bedri2017earbit,bedri2015wearable,bi2017toward}.
Eating as an activity is a very subtle motion. It involves repeated hand movement to the mouth which varies vastly depending on the eating habits and the food consumed. 
Many studies \cite{althubaiti2016information, bedri2017earbit, bedri2015wearable, bi2017toward, morshed2020real} have proposed many wrist based wearable systems to automatically monitor food consumption yet most of them are either based on special custom systems or are tested in a controlled environment. While other monitoring wearable try to match one of the actions that occur during food intake; e.g., hand movement while bringing the food to the mouth, biting and chewing, or swallowing \cite{dong2013detecting}. However, there are lots of proxy movements in daily living that can create false positives for such detection methods.

One of the key challenges in a fully automated food intake monitoring system is to identify whether the eating has happened or not within a given time frame. Past works have tried to solve this problem using training an eating moment recognition method on carefully curated in-lab datasets and then testing upon semi-controlled wild datasets \cite{thomaz2015practical}. 
While these methods have shown robust accuracies, they are still limited by the amount of lab data available to them for training. Our work illustrates a potential solution to this problem in the form of an existing work IMUTube \cite{kwon2020imutube}, while also understanding various caveats of its working.
\thomas{Structure is ok -- if we agree on actually having a dedicated eating section in here (I thought we wanted to broaden the scope? Let's discuss.) -- but it needs serious proofreading and copy-editing. Grammar is a bit all over the place.}



==> sections/result/prev/_tmp.tex <==
% keep text from 10/02/2022
\section{Results}

\input{figure/msi_corr}

\subsection{Correlation Analysis between MSI and rMSI}

Here, we first validate how the proposed MSI correlates with the motion subtlety actually measured from real IMU dataset, rMSI. 
From 17 activity classes included in the benchmark daily activity datasets~\cite{inproceedings}, we collect the mode of MSI distribution for each class samples, MSI$_c$, from curated video dataset.
The modes of rMSI distribution for each class are collected directly from real IMU datasets.
\autoref{fig:msi_corr} shows the correlation analysis between MSI and rMSI.
Pearson correlation analysis demonstrated statistically strong correlation between two values ($r=0.746$, $p\leq 0.006$) across 17 activities validating that MSI can effectively quantify subtle motions from human activities in the video.

\subsection{Daily Activity Classification}

\autoref{tab:results} shows the classification performance measured in F1 score for daily activity and eating recognition tasks.

\subsubsection{Effect of Real IMU Data Scale}

We have simulated two cases for the application of virtual IMU data for the activities with subtle motions: the availability of small and large scale real IMU dataset.
For the cases with small IMU dataset, we used 20\% of real IMU data available in the training datasets, and for the cases with large scale real IMU dataset, we used all (100\%) real IMU dataset available.

The use of virtual IMU data was partially successful with those two cases.
Virtual IMU data could only improve the classification performance statistically significantly when small real IMU data was available.
For daily activity classification, compared to when only using 20\% of real IMU dataset, using curated and in-the-wild videos, relatively improved 4.2\% and 2.3\% F1 scores, respectively.
As expected, model trained with virtual IMU data from curated video outperformed that from in-the-wild video, which was consistent with the previous studies~\cite{kwon2021approaching}.

When we had sufficient number of real IMU dataset, the effect of using virtual IMU data was only marginal statistically showing very similar performances compared to real IMU dataset.
We consider that the model relied heavily on real IMU data to capture very detailed movement patterns for the classification tasks as the movements in virtual IMU data were either too simplistic to capture discriminative patterns.
IMUTube is designed to capture substantional movements using 3D joint motion tracking techniques, which tracks approximated estimation of joint locations that is limited in capturing subtle movements in the wrist.

\subsubsection{Effect of Using MSI}

The proposed method could statistically significantly improve the model by additionally quantifying the motion subtlety index for both virtual and real IMU data to select most effective virtual IMU data segements for model traning.
When small real IMU dataset is used, using MSI could improve relative 3$\%$ and \hl{X\%} when using virtual IMU data from curated and in-the-wild videos, respectively.
Similarly, when sufficiently large real IMU dataset was available, using MSI for being selectively in choosing virtual IMU data, could improve relative 2\% and \hl{X\%} of F1 score for daily activity classification tasks.

\input{tables/results}

\subsection{Eating Moment Recognition}

\subsubsection{Effect of Real IMU Data Scale}
% 20\% dataset
\hyeok{Waiting for 20\% results from Zikang}

Much to our surprise, virtual IMU data was very effective for eating specific activity classification task.
Even when using all real IMU dataset, unlikely from the daily activity classification task, adding virtual IMU data have significantly improved the performance of the model.
The baseline model using only real IMU data achieved 71.5\% F1-score, and our model trained with the curated virtual IMU dataset improved that to 79.94\%.
The in-the-wild-scenario increased the recognition performance by 5.9\% to 77.45\%.
We suspect this improvement came from the virtual IMU data containing wide range of fine-grained eating motions collected from videos for varying utensils or food types.
(For the case of daily activity dataset, we only collected eating video for "eating sandwich" class, which were more limited in sample size and variations in motions)

\subsubsection{Effect of Using MSI}

\hyeok{Waiting for Zikang's results}

==> sections/result/prev/_tmp2.tex <==
\section{Results}

\input{tables/results_no_msi}

Before discussing the classification performance changes with respect to MSI, we first demonstrate the classification results for daily activity and eating recognition tasks with the standard approach used with virtual IMU dataset. \thomas{Why?}\hyeok{To first to show that IMUTube fails for these classes}
Here, we additionally study the effect of virtual IMU data regarding the availability of real IMU dataset. \thomas{Why? That was done in previous papers.}\hyeok{So, using virtual IMU dataset was only hurting when using 100\% real IMU data. We wanted to find the point where at least virtual IMU data gives benefit and analyze there.}
In \autoref{tab:results}, we reported classification results either using 20\% or 100\% of real IMU dataset available in each dataset as we could observe different behaviors.
More detailed analysis on the effect of real IMU data scale is conducted in \autoref{sec:msi_group_real_size}.

\subsection{Daily Activity Classification}

This dataset includes activities that invovles very subtle motions such as writing, reading, or drawing activities in daily living.
For such activity, the use of virtual IMU data was partially successful, where virtual IMU data could only improve the classification performance statistically significantly when small real IMU data was available.
For daily activity classification, compared to when only using 20\% of real IMU dataset, using curated and in-the-wild videos, relatively improved 4.2\% and 2.3\% F1 scores, respectively.
As expected, model trained with virtual IMU data from curated video outperformed that from in-the-wild video, which was consistent with the previous studies~\cite{kwon2021approaching}.
In \autoref{sec:msi_f1_all}, we discuss more in detail how F1 score changes according to MSI values for the virtual IMU data used for model training.

When we had sufficient number of real IMU dataset, using virtual IMU data demonstrated to be statistically insignificant and resulted in very similar performances compared to real IMU dataset.
We consider that the model relied heavily on real IMU data to capture very detailed movement patterns for the classification tasks as the movements in virtual IMU data were either too simplistic to capture discriminative patterns.
IMUTube is designed to capture substantial movements using 3D joint motion tracking techniques, which tracks approximated estimation of joint locations that is limited in capturing subtle movements in the wrist.

\subsection{Eating Moment Recognition}

\hyeok{Waiting for 20\% results from Zikang}

Much to our surprise, virtual IMU data was very effective for eating specific activity classification task.
Even when using all real IMU dataset, differently from the daily activity classification task, adding virtual IMU data have significantly improved the performance of the model.
The baseline model using only real IMU data achieved 71.5\% F1-score, and our model trained with the curated virtual IMU dataset improved that to 79.94\%.
The in-the-wild-scenario increased the recognition performance by 5.9\% to 77.45\%.
We suspect this improvement came from the virtual IMU data containing wide range of fine-grained eating motions collected from videos for varying utensils or food types.
Daily activity classification dataset only included "eating sandwich" class, which were more limited in hand and arm motions compared to other kinds of eating activities.

==> tables/results.tex <==
\begin{table}[t]
    \centering
    \caption{Model performances for daily activity and eating classification tasks.
    Daily activity classification is evaluated with mean F1 score, and eating classification is evaluated with binary F1 score.
    For daily activity classification, we test for two different cases when real IMU data is sparse or sufficiently large.
    For daily activity with very subtle motions, virtual IMU data was useful when only small number of real IMU data was available.
    The best performance within a experiment setting was highlighted with \textbf{bold}.
    }
    \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{c|c|c|c|c}
          Task & Real (\%) & Virtual & MSI & F1 score \\
         \hline\hline
         \multirow{10}{*}{Daily Activity~\cite{inproceedings}} 
         & \multirow{5}{*}{20} & - & - & $0.3066 \pm 0.0009$\\
         \cline{3-5}
         & & Curated & - & $0.3194 \pm 0.0017$ \\
         \cline{3-5}
         & & In-the-wild & - & $0.3137 \pm 0.0011$\\
         \cline{3-5}
         & & Curated & \checkmark & $\textbf{0.3290} \pm 0.0016$ \\
         \cline{3-5}
         & & In-the-wild & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \hhline{~====}
         & \multirow{5}{*}{100} & - & - & $\textbf{0.4769} \pm 0.0008$\\
         \cline{3-5}
         & & Curated & & $0.4621 \pm 0.0007$ \\
         \cline{3-5}
         & & In-the-wild & & $0.4715 \pm 0.0011$\\
         \cline{3-5}
         & & Curated & \checkmark & $0.4712 \pm 0.0012$ \\
         \cline{3-5}
         & & In-the-wild & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \hline\hline
         \multirow{10}{*}{Eating~\cite{thomaz2015practical}} 
         & \multirow{5}{*}{20} & - & - & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-5}
         &  & Curated & - & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-5}
         &  & In-the-wild & - & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-5}
         &  & Curated & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-5}
         &  & In-the-wild & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \hhline{~====}
         & \multirow{5}{*}{100} & - & - & $0.7150 \pm 0.0000$\\
         \cline{3-5}
         & & Curated & - & $\textbf{0.7994} \pm 0.0000$\\
         \cline{3-5}
         & & In-the-wild & - & $0.7745 \pm 0.0000$\\
         \cline{3-5}
         & & Curated & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-5}
         & & In-the-wild & \checkmark & \hl{$0.0000 \pm 0.0000$}\\
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:results}
\end{table}

==> tables/results_no_msi.tex <==
\begin{table}[t]
    \centering
    \caption{Model performances for daily activity and eating classification tasks.
    Daily activity classification is evaluated with mean F1 score, and eating classification is evaluated with binary F1 score.
    For daily activity classification, we test for two different cases when real IMU data is sparse or sufficiently large.
    For daily activity with very subtle motions, virtual IMU data was useful when only small number of real IMU data was available.
    The best performance within a experiment setting was highlighted with \textbf{bold}.
    }
    \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{c|c|c|c}
          Task & Real (\%) & Virtual & F1 score \\
         \hline\hline
         \multirow{6}{*}{Daily Activity~\cite{inproceedings}} 
         & \multirow{3}{*}{20} & - & $0.3066 \pm 0.0009$\\
         \cline{3-4}
         & & Curated & $\textbf{0.3194} \pm 0.0017$ \\
         \cline{3-4}
         & & In-the-wild & $0.3137 \pm 0.0011$\\
         \cline{3-4}
         \hhline{~===}
         & \multirow{3}{*}{100} & - & $\textbf{0.4769} \pm 0.0008$\\
         \cline{3-4}
         & & Curated & $0.4621 \pm 0.0007$ \\
         \cline{3-4}
         & & In-the-wild & $0.4715 \pm 0.0011$\\
         \cline{3-4}
         \hline\hline
         \multirow{6}{*}{Eating~\cite{thomaz2015practical}} 
         & \multirow{3}{*}{20} & - & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-4}
         &  & Curated & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-4}
         &  & In-the-wild & \hl{$0.0000 \pm 0.0000$}\\
         \cline{3-4}
         \hhline{~===}
         & \multirow{3}{*}{100} & - & $0.7150 \pm 0.0000$\\
         \cline{3-4}
         & & Curated & $\textbf{0.7994} \pm 0.0000$\\
         \cline{3-4}
         & & In-the-wild & $0.7745 \pm 0.0000$\\
         \cline{3-4}
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:results}
\end{table}
